The Challenges of Crowd Workers in Rural and Urban America

Crowd work has the potential of helping the financial recovery of regions traditionally plagued by a lack of economic opportunities, e.g., rural areas. However, we currently have limited information about the challenges facing crowd work-ers from rural and super rural areas as they struggle to make a living through crowd work sites. This paper examines the challenges and advantages of rural and super rural AmazonMechanical Turk (MTurk) crowd workers and contrasts them with those of workers from urban areas. Based on a survey of421 crowd workers from differing geographic regions in theU.S., we identified how across regions, people struggled with being onboarded into crowd work. We uncovered that despite the inequalities and barriers, rural workers tended to be striving more in micro-tasking than their urban counterparts. We also identified cultural traits, relating to time dimension and individualism, that offer us an insight into crowd workers and the necessary qualities for them to succeed on gig platforms. We finish by providing design implications based on our findings to create more inclusive crowd work platforms and tools

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release


==> backuptext.tex <==

Through our analysis we identified that workers spent daily almost the same amount of time on paid labor than what they spent on invisible labor. Given this, we argue it is important to 
Next, we calculated the hourly wage of workers in our study based on the amount of time they worked on MTurk and their total earnings for that day. 
{\tiny {Work Times}}  & {\tiny Total time workers invested on completing HITs per day}&{\tiny 219 min}\\
\rowcolor{LightGreen}








\begin{table}[t]
\begin{center}
\begin{tabular}{ |p{14mm}|p{43mm}|p{7mm}| }
\hline
%\multicolumn{3}{ |c| }{} \\
%\hline
%Variable & Value \\ \hline
\multirow{4}{*}{\tiny {\bf Tasks \& Workers}} 
& {\tiny Total number of tasks} & {\tiny41,586}\\
& {\tiny Total number of workers} &{\tiny98}\\
&&\\
 & {\tiny Min tasks per worker} &{\tiny1}\\
 & {\tiny Median tasks per worker}&{\tiny186}\\
 & {\tiny Max tasks per worker}&{\tiny 3,187}\\
  &&\\
  & {\tiny Min tasks per day} &{\tiny 0}\\
 & {\tiny Median tasks per day}&{\tiny 32}\\
 & {\tiny Max tasks per day}&{\tiny 1,168}\\
 \hline
 \multirow{2}{*}{\tiny {\bf Work Times}} 
& {\tiny Total time on HITs per day}&{\tiny 219 min}\\
& {\tiny Min time on HITs per day}&{\tiny 0 min}\\
& {\tiny Median time on HITs per day}&{\tiny 1.25 hrs}\\
& {\tiny Max time on HITs per day}&{\tiny XX min}\\
 &&\\
&{\tiny Total time on invisible labor per day}&{\tiny 139 min}\\
&{\tiny Min time on invisible labor per day}&{\tiny 0 min}\\
&{\tiny Median time on invisible labor per day}&{\tiny 1.19 hrs}\\
&{\tiny Max time on invisible labor per day}&{\tiny XX min}\\
\hline
\multirow{3}{*}{\tiny {\bf Earnings}} 
& {\tiny Min earnings per worker (total week)} &{\tiny 0.92\cent}\\
 & {\tiny Median earnings per worker (total week)}&{\tiny \$55.46}\\
 & {\tiny Max earnings per worker (total week)}&{\tiny \$640.19}\\
 &&\\
 
 & {\tiny Min earnings per worker per day} &{\tiny 0.01\cent}\\
 & {\tiny Median earnings per worker per day}&{\tiny\$8.65}\\
 & {\tiny Max earnings per worker per day}&{\tiny\$178.62}\\
 &&\\
 
 & {\tiny Median Hourly wage with invisible labor}&{\tiny\$1.74}\\
 & {\tiny Median Hourly wage without invisible labor}&{\tiny\$4.08}\\
\hline
\multirow{3}{*}{\tiny {\bf Multi-Tasking}} 
& {\tiny Percentage of workers who multi-task} &{\tiny 98\%}\\
&&\\
& {\tiny Min number of tasks done in multi-tasking}&{\tiny XX}\\
 & {\tiny Median number of tasks done in multi-tasking}&{\tiny 144}\\
  & {\tiny Max number of tasks done in multi-tasking}&{\tiny XX}\\
  &&\\
 & {\tiny Min number of batches done in multi-tasking}&{\tiny XX}\\
 & {\tiny Median number of batches done in multi-tasking}&{\tiny 18}\\
 & {\tiny Max number of batches done in multi-tasking}&{\tiny XX}\\
  &&\\
 & {\tiny Min number of tasks in a batch}&{\tiny XX}\\
 & {\tiny Median number of tasks in a batch}&{\tiny 8}\\
 & {\tiny Max number of tasks in a batch}&{\tiny XX}\\
 \hline
\end{tabular}
\caption[Table caption text]{Summary of statistics in our study with regard to: a) tasks workers did; b) the time they invested in working; c) workers' earnings; and d) their multi-tasking information.}
\label{table:stats}
\end{center}
\end{table}






















Based on the amount of time that workers spent on MTurk conducting different activities and based on the total earnings that they made within that time period, 












they accepted to work on a HIT, but before finishing and submitting the HIT,  they accepted to work on another HIT. 

%\section{Formatting Requirements in Brief}
%We need source and PDF files that can be used in a variety of ways and can be output on a variety of devices. The design and appearance of the paper is strictly governed by the aaai style file (aaai20.sty). 
%\textbf{You must not make any changes to the aaai style file, nor use any commands, packages, style files, or macros within your own paper that alter that design, including, but not limited to spacing, floats, margins, fonts, font size, and appearance.} AAAI imposes requirements on your source and PDF files that must be followed. Most of these requirements are based on our efforts to standardize conference manuscript properties and layout. All papers submitted to AAAI for publication will be recompiled for standardization purposes. Consequently, every paper submission must comply with the following requirements:

%\begin{quote}
%\begin{itemize}
%\item Your .tex file must compile in PDF\LaTeX{} --- ( you may not include .ps or .eps figure files.)
%\item All fonts must be embedded in the PDF file --- including includes your figures.
%\item Modifications to the style file, whether directly or via commands in your document may not ever be made, most especially when made in an effort to avoid extra page charges or make your paper fit in a specific number of pages.
%\item No type 3 fonts may be used (even in illustrations).
%\item You may not alter the spacing above and below captions, figures, headings, and subheadings.
%\item You may not alter the font sizes of text elements, footnotes, heading elements, captions, or title information (for references and mathematics, please see the the limited exceptions provided herein).
%\item You may not alter the line spacing of text.
%\item Your title must follow Title Case capitalization rules (not sentence case).
%\item Your .tex file must include completed metadata to pass-through to the PDF (see PDFINFO below)
%\item \LaTeX{} documents must use the Times or Nimbus font package (you may not use Computer Modern for the text of your paper).
%\item No \LaTeX{} 209 documents may be used or submitted.
%\item Your source must not require use of fonts for non-Roman alphabets within the text itself. If your paper includes symbols in other languages (such as, but not limited to, Arabic, Chinese, Hebrew, Japanese, Thai, Russian and other Cyrillic languages), you must restrict their use to bit-mapped figures. Fonts that require non-English language support (CID and Identity-H) must be converted to outlines or 300 dpi bitmap or removed from the document (even if they are in a graphics file embedded in the document). 
%\item Two-column format in AAAI style is required for all papers.
%\item The paper size for final submission must be US letter without exception.
%\item The source file must exactly match the PDF.
%\item The document margins may not be exceeded (no overfull boxes).
%\item The number of pages and the file size must be as specified for your event.
%\item No document may be password protected.
%\item Neither the PDFs nor the source may contain any embedded links or bookmarks (no hyperref or navigator packages).
%\item Your source and PDF must not have any page numbers, footers, or headers (no pagestyle commands).
%\item Your PDF must be compatible with Acrobat 5 or higher.
%\item Your \LaTeX{} source file (excluding references) must consist of a \textbf{single} file (use of the ``input" command is not allowed.
%\item Your graphics must be sized appropriately outside of \LaTeX{} (do not use the ``clip" or ``trim'' command) .
%\end{itemize}
%\end{quote}

%If you do not follow these requirements, you will be required to correct the deficiencies and resubmit the paper. A resubmission fee will apply.

%\section{What Files to Submit}
%You must submit the following items to ensure that your paper is published:
%\begin{itemize}
%\item A fully-compliant PDF file that includes PDF metadata.
%\item Your \LaTeX{} source file submitted as a \textbf{single} .tex file (do not use the ``input" command to include sections of your paper --- every section must be in the single source file). (The only allowable exception is .bib file, which should be included separately). 
%\item The bibliography (.bib) file(s).
%\item Your source must compile on our system, which includes only standard \LaTeX{} 2019 TeXLive support files. 
%\item Only the graphics files used in compiling paper.
%\item The \LaTeX{}-generated files (e.g. .aux,  .bbl file, PDF, etc.).
%\end{itemize}

%Your \LaTeX{} source will be reviewed and recompiled on our system (if it does not compile, you will be required to resubmit, which will incur fees). \textbf{Do not submit your source in multiple text files.} Your single \LaTeX{} source file must include all your text, your bibliography (formatted using aaai.bst), and any custom macros. 

%Your files should work without any supporting files (other than the program itself) on any computer with a standard \LaTeX{} distribution. 

%\textbf{Do not send files that are not actually used in the paper.} We don't want you to send us any files not needed for compiling your paper, including, for example, this instructions file, unused graphics files, style files, additional material sent for the purpose of the paper review, and so forth.

%\textbf{Do not send supporting files that are not actually used in the paper.} We don't want you to send us any files not needed for compiling your paper, including, for example, this instructions file, unused graphics files, style files, additional material sent for the purpose of the paper review, and so forth.

%\textbf{Obsolete style files.} The commands for some common packages (such as some used for algorithms), may have changed. Please be certain that you are not compiling your paper using old or obsolete style files. 
%\textbf{Final Archive.} Place your PDF and source files in a single archive which should be compressed using .zip. The final file size may not exceed 10 MB.
%Name your source file with the last (family) name of the first author, even if that is not you.


%\section{Using \LaTeX{} to Format Your Paper}

%The latest version of the AAAI style file is available on AAAI's website. Download this file and place it in the \TeX\ search path. Placing it in the same directory as the paper should also work. You must download the latest version of the complete AAAI Author Kit so that you will have the latest instruction set and style file.

%\subsection{Document Preamble}

%In the \LaTeX{} source for your paper, you \textbf{must} place the following lines as shown in the example in this subsection. This command set-up is for three authors. Add or subtract author and address lines as necessary, and uncomment the portions that apply to you. In most instances, this is all you need to do to format your paper in the Times font. The helvet package will cause Helvetica to be used for sans serif. These files are part of the PSNFSS2e package, which is freely available from many Internet sites (and is often part of a standard installation).

%Leave the setcounter for section number depth commented out and set at 0 unless you want to add section numbers to your paper. If you do add section numbers, you must uncomment this line and change the number to 1 (for section numbers), or 2 (for section and subsection numbers). The style file will not work properly with numbering of subsubsections, so do not use a number higher than 2.

%If (and only if) your author title information will not fit within the specified height allowed, put \textbackslash setlength \textbackslash titlebox{2.5in} in your preamble. Increase the height until the height error disappears from your log. You may not use the \textbackslash setlength command elsewhere in your paper, and it may not be used to reduce the height of the author-title box.

%\subsubsection{The Following Must Appear in Your Preamble}
%\begin{quote}
%\begin{scriptsize}\begin{verbatim}
%\documentclass[letterpaper]{article}
%\usepackage{aaai20}
%\usepackage{times}
%\usepackage{helvet}
%\usepackage{courier}
%\usepackage[hyphens]{url} 
%\usepackage{graphicx}
%\urlstyle{rm}
%\def\UrlFont{\rm}
%\usepackage{graphicx}
%\frenchspacing
%\setlength{\pdfpagewidth}{8.5in}
%\setlength{\pdfpageheight}{11in}
%% Add additional packages here, but check 
%% the list of disallowed packages 
%% (including, but not limited to
%% authblk, caption, CJK, float, fullpage, geometry, 
%% hyperref, layout, nameref, natbib, savetrees, 
%% setspace, titlesec, tocbibind, ulem)
%% and illegal commands provided in the 
%% common formatting errors document
%% included in the  Author Kit before doing so. 
%
% PDFINFO
% You are required to complete the following
% for pass-through to the PDF. 
% No LaTeX commands of any kind may be
% entered. The parentheses and spaces 
% are an integral part of the 
% pdfinfo script and must not be removed.
%
%\pdfinfo{
%/Title (Type Your Paper Title Here in Mixed Case)
%/Author (John Doe, Jane Doe)
%/Keywords (Input your keywords in this optional area)
%}
%
% Section Numbers
% Uncomment if you want to use section numbers
% and change the 0 to a 1 or 2
% \setcounter{secnumdepth}{0}

% Title and Author Information Must Immediately Follow
% the pdfinfo within the preamble
%
%\title{Title}\\
%\author\{Author 1 \ and Author 2\\
%Address line\\
%Address line\\
%\ And\\
%Author 3\\
%Address line\\
%Address line
%}\\
%\end{verbatim}\end{scriptsize}
%\end{quote}

%\subsection{Preparing Your Paper}

%After the preamble above, you should prepare your paper as follows:
%\begin{quote}
%\begin{scriptsize}\begin{verbatim}
%
%\begin{document}
%\maketitle
%\begin{abstract}
%%...
%\end{abstract}\end{verbatim}\end{scriptsize}
%\end{quote}

%\subsubsection{The Following Must Conclude Your Document}
%\begin{quote}
%\begin{scriptsize}\begin{verbatim}
% References and End of Paper
% These lines must be placed at the end of your paper
%\bibliography{Bibliography-File}
%\bibliographystyle{aaai}
%\end{document}
%\end{verbatim}\end{scriptsize}
%\end{quote}

%\subsection{Inserting Document Metadata with %\LaTeX{}}
%PDF files contain document summary information that %enables us to create an Acrobat index (pdx) file, and %also allows search engines to locate and present your %paper more accurately. \textit{Document metadata for %author and title are REQUIRED.} You may not apply any %script or macro to implementation of the title, %author, and metadata information in your paper.

%\textit{Important:} Do not include \textit{any} \LaTeX{} code or nonascii characters (including accented characters) in the metadata. The data in the metadata must be completely plain ascii. It may not include slashes, accents, linebreaks, unicode, or any \LaTeX{} commands. Type the title exactly as it appears on the paper (minus all formatting). Input the author names in the order in which they appear on the paper (minus all accents), separating each author by a comma. You may also include keywords in the optional Keywords field.

%\begin{quote}
%\begin{scriptsize}\begin{verbatim}
%\begin{document}\\
%\maketitle\\
%...\\
%\bibliography{Bibliography-File}\\
%\bibliographystyle{aaai}\\
%\end{document}\\
%\end{verbatim}\end{scriptsize}
%\end{quote}

%\subsection{Commands and Packages That May Not Be Used}
%\begin{table*}[t]
%\centering
%\caption{Commands that must not be used}\smallskip
%\begin{tabular}{l|l|l|l}
%\textbackslash abovecaption & 
%\textbackslash abovedisplay & 
%\textbackslash addevensidemargin & 
%\textbackslash addsidemargin \\ 
%\textbackslash addtolength & 
%\textbackslash baselinestretch & 
%\textbackslash belowcaption & 
%\textbackslash belowdisplay \\ 
%\textbackslash break &
%\textbackslash clearpage & 
%\textbackslash clip & 
%\textbackslash columnsep \\ 
%\textbackslash float & 
%\textbackslash input & 
%\textbackslash input & 
%\textbackslash linespread \\ 
%\textbackslash newpage &
%\textbackslash pagebreak & 
%\textbackslash renewcommand & 
%\textbackslash setlength \\ 
%\textbackslash text height & 
%\textbackslash tiny & 
%\textbackslash top margin & 
%\textbackslash trim \\ 
%\textbackslash vskip\{- & 
%\textbackslash vspace\{- \\ 
%\end{tabular}
%}
%\label{table1}
%\end{table*}

%\begin{table}[t]
%\caption{LaTeX style packages that must not be %used.}\smallskip
%\centering
%\resizebox{.95\columnwidth}{!}{
%\smallskip\begin{tabular}{l|l|l|l}
%authblk & babel & caption & cjk\\
%dvips & epsf & epsfig & euler\\
%float & fullpage & geometry & graphics\\
%hyperref & layout & linespread & lmodern\\
%maltepaper & natbib & navigator & pdfcomment\\
%pgfplots & psfig & pstricks & t1enc \\
%titlesec & tocbind & ulem\\
%\end{tabular}
%\label{table2}
%\end{table}%

%There are a number of packages, commands, scripts, and macros that are incompatable with aaai20.sty. The common ones are listed in tables \ref{table1} and \ref{table2}. Generally, if a command, package, script, or macro alters floats, margins, fonts, sizing, linespacing, or the presentation of the references and citations, it is unacceptable. Note that negative vskip and vspace may not be used except in certain rare occurances, and may never be used around tables, figures, captions, sections, subsections, subsections, or references. 


%\subsection{Page Breaks}
%For your final camera ready copy, you must not use any page break commands. References must flow directly after the text without breaks. Note that some conferences require references to be on a separate page during the review process. AAAI Press, however, does not require this condition for the final paper. 


%\subsection{Paper Size, Margins, and Column Width}
%Papers must be formatted to print in two-column format on 8.5 x 11 inch US letter-sized paper. The margins must be exactly as follows: 
%\begin{itemize}
%\item Top margin: .75 inches
%\item Left margin: .75 inches
%\item Right margin: .75 inches
%\item Bottom margin: 1.25 inches
%\end{itemize} 


%The default paper size in most installations of \LaTeX{} is A4. However, because we require that your electronic paper be formatted in US letter size, the preamble we have provided includes commands that alter the default to US letter size. Please note that using any other package to alter page size (such as, but not limited to the Geometry package) will result in your final paper being returned to you for correction and payment of a resubmission fee. 


%\subsubsection{Column Width and Margins.}
%To ensure maximum readability, your paper must include two columns. Each column should be 3.3 inches wide (slightly more than 3.25 inches), with a .375 inch (.952 cm) gutter of white space between the two columns. The aaai20.sty file will automatically create these columns for you. 

%\subsection{Overlength Papers}
%If your paper is too long, turn on \textbackslash frenchspacing, which will reduce the space after periods. Next, shrink the size of your graphics. Use \textbackslash centering instead of \textbackslash begin\{center\} in your figure environment. For mathematical environments, you may reduce fontsize {\bf but not below 6.5 point}. You may also alter the size of your bibliography and tables by inserting \textbackslash fontsize\{9.5pt\}\{10.5pt\} \textbackslash selectfont
%right before the bibliography (the minimum size is \textbackslash fontsize\{9.0pt\}\{10.0pt\}. You may not use any commands that further reduce point size. Be careful when scaling tables and figures. Tables that do not fit in a single column, even after the font size reduction to 9 point, must be placed across double columns. If your table won't fit within the margins even in double columns, you must split it. We will not accept single (or double) column tables that have been scaled to anything below 9 point. 


%Commands that alter page layout are forbidden. These include \textbackslash columnsep, \textbackslash topmargin, \textbackslash topskip, \textbackslash textheight, \textbackslash textwidth, \textbackslash oddsidemargin, and \textbackslash evensizemargin (this list is not exhaustive). If you alter page layout, you will be required to pay the page fee \textit{plus} a reformatting fee. Other commands that are questionable and may cause your paper to be rejected include \textbackslash parindent, and \textbackslash parskip. Commands that alter the space between sections are forbidden. The title sec package is not allowed. Regardless of the above, if your paper is obviously ``squeezed" it is not going to to be accepted. Options for reducing the length of a paper include reducing the size of your graphics, cutting text, or paying the extra page charge (if it is offered). 

%\subsection{Figures}
%Your paper must compile in PDF\LaTeX{}. Consequently, all your figures must be .jpg, .png, or .pdf. You may not use the .gif (the resolution is too low), .ps, or .eps file format for your figures.

%If you normally create your figures using pgfplots, please create the figures first, and then import them as pdfs with proper bounding boxes, as the bounding and trim boxes created by pfgplots are fragile, and not valid.

%When you include your figures, you must crop them \textbf{outside} of \LaTeX{}. The command \textbackslash includegraphics*[clip=true, viewport 0 0 10 10]{...} might result in a PDF that looks great, but the image is \textbf{not really cropped.} The full image can reappear (and obscure whatever it is overlapping) when page numbers are applied or color space is standardized. Figures \ref{fig1}, and \ref{fig2} display some unwanted results that often occur.

%Do not use minipage to group figures. Additionally, the font and size of figure captions must be 10 point roman. Do not make them smaller, bold, or italic. (Individual words may be italicized if the context requires differentiation.)

%\begin{figure}[t]
%\%centering
%\includegraphics[width=0.9\columnwidth]{figure1} % Reduce the figure size so that it is slightly narrower than the column. Don't use precise values for figure width.This setup will avoid overfull boxes. 
%\caption{Using the trim and clip commands produces fragile layers that can result in disasters (like this one from an actual paper) when the color space is corrected or the PDF combined with others for the final proceedings. Crop your figures properly in a graphics program -- not in LaTeX}
%\label{fig1}
%\end{figure}

%\begin{figure*}[t]
%\centering
%\includegraphics[width=0.8\textwidth]{figure2} % %Reduce the figure size so that it is slightly %narrower than the column.
%\caption{Adjusting the bounding box instead of %actually removing the unwanted data resulted multiple %layers in this paper. It also needlessly increased %the PDF size. In this case, the size of the unwanted %layer doubled the paper's size, and produced the %following surprising results in final production. %Crop your figures properly in a graphics program. %Don't just alter the bounding box.}
%\label{fig2}
%\end{figure*}%

% Using the \centering command instead of \begin{center} ... \end{center} will save space
% Positioning your figure at the top of the page will save space and make the paper more readable
% Using 0.95\columnwidth in conjunction with the 

%\subsection{Type Font and Size}
%Your paper must be formatted in Times Roman or Nimbus. We will not accept papers formatted using Computer Modern or Palatino or some other font as the text or heading typeface. Sans serif, when used, should be Courier. Use Symbol or Lucida or Computer Modern for \textit{mathematics only. } 

%Do not use type 3 fonts for any portion of your paper, including graphics. Type 3 bitmapped fonts are designed for fixed resolution printers. Most print at 300 dpi even if the printer resolution is 1200 dpi or higher. They also often cause high resolution imagesetter devices and our PDF indexing software to crash. Consequently, AAAI will not accept electronic files containing obsolete type 3 fonts. Files containing those fonts (even in graphics) will be rejected. 

%Fortunately, there are effective workarounds that will prevent your file from embedding type 3 bitmapped fonts. The easiest workaround is to use the required times, helvet, and courier packages with \LaTeX{}2e. (Note that papers formatted in this way will still use Computer Modern for the mathematics. To make the math look good, you'll either have to use Symbol or Lucida, or you will need to install type 1 Computer Modern fonts --- for more on these fonts, see the section ``Obtaining Type 1 Computer Modern.")

%If you are unsure if your paper contains type 3 fonts, view the PDF in Acrobat Reader. The Properties/Fonts window will display the font name, font type, and encoding properties of all the fonts in the document. If you are unsure if your graphics contain type 3 fonts (and they are PostScript or encapsulated PostScript documents), create PDF versions of them, and consult the properties window in Acrobat Reader. 

%The default size for your type must be ten-point with twelve-point leading (line spacing). Start all pages (except the first) directly under the top margin. (See the next section for instructions on formatting the title page.) Indent ten points when beginning a new paragraph, unless the paragraph begins directly below a heading or subheading.


%\subsubsection{Obtaining Type 1 Computer Modern for \LaTeX{}.}

%If you use Computer Modern for the mathematics in your paper (you cannot use it for the text) you may need to download type 1 Computer fonts. They are available without charge from the American Mathematical Society:
%http://www.ams.org/tex/type1-fonts.html. 

%\subsubsection{Nonroman Fonts}
%If your paper includes symbols in other languages (such as, but not limited to, Arabic, Chinese, Hebrew, Japanese, Thai, Russian and other Cyrillic languages), you must restrict their use to bit-mapped figures. 

%\subsection{Title and Authors}
%Your title must appear in mixed case (nouns, pronouns, and verbs are capitalized) near the top of the first page, centered over both columns in sixteen-point bold type (twenty-four point leading). This style is called ``mixed case," which means that means all verbs (including short verbs like be, is, using,and go), nouns, adverbs, adjectives, and pronouns should be capitalized, (including both words in hyphenated terms), while articles, conjunctions, and prepositions are lower case unless they directly follow a colon or long dash. Author's names should appear below the title of the paper, centered in twelve-point type (with fifteen point leading), along with affiliation(s) and complete address(es) (including electronic mail address if available) in nine-point roman type (the twelve point leading). (If the title is long, or you have many authors, you may reduce the specified point sizes by up to two points.) You should begin the two-column format when you come to the abstract. 

%\subsubsection{Formatting Author Information}
%Author information can be set in a number of different styles, depending on the number of authors and the number of affiliations you need to display. In formatting your author information, however, you may not use a table nor may you employ the \textbackslash authorblk.sty package. For several authors from the same institution, please just separate with commas:

%\begin{quote}\begin{scriptsize}\begin{verbatim}
%\author{Author 1, ... Author n\\ 
%Address line \\ ... \\ Address line}
%\end{verbatim}\end{scriptsize}\end{quote}

%\noindent If the names do not fit well on one line use:

%\begin{quote}\begin{scriptsize}\begin{verbatim}
%\author{Author 1} ... \\
%{\bf \Large Author ... Author}\\ 
%Address line \\ ... \\ Address line
%}
%\end{verbatim}\end{scriptsize}\end{quote}

%\noindent For two (or three) authors from different institutions, use \textbackslash And:

%\begin{quote}\begin{scriptsize}\begin{verbatim}
%\author{Author 1\\ Address line \\ ... \\ Address line 
%\And ... \And Author n\\
%Address line\\ ... \\ Address line}
%\end{verbatim}\end{scriptsize}\end{quote}

%\noindent To start a separate ``row" of authors, use %\textbackslash AND:

%If the title and author information does not fit in the area allocated, place
%\textbackslash setlength\textbackslash titlebox\{\textit{height}\}
%after the \textbackslash documentclass line where \{\textit{height}\} is 2.5in or greater. (This one of the only allowable uses of the setlength command. Check with AAAI Press before using it elsewhere.)

%\subsubsection{Formatting Author Information --- Alternative Method}
%If your paper has a large number of authors from different institutions, you may use the following alternative method for displaying the author information.

%\begin{quote}\begin{scriptsize}\begin{verbatim}
%\author{AuthorOne},\textsuperscript{\rm 1} 
%AuthorTwo,\textsuperscript{\rm 2}
%AuthorThree,\textsuperscript{\rm 3}
%\\bf \Large AuthorFour,\textsuperscript{\rm 4} 
%AuthorFive, \textsuperscript{\rm 5}\\
%\textsuperscript{\rm 1}AffiliationOne, 
%\textsuperscript{\rm 2}AffiliationTwo, 
%\textsuperscript{\rm 3}AffiliationThree\\
%\textsuperscript{\rm 4}AffiliationFour, 
%\textsuperscript{\rm 5}AffiliationFive 
%\{email, email\}@affiliation.com,
%e%mail@affiliation.com,
%email@affiliation.com, 
%email@affiliation.com
%\end{verbatim}\end{scriptsize}\end{quote}%

%Note that you should break the author list before it extends into the right column margin. Put a line break, followed by   \textbackslash bf  \textbackslash Large to put the second line of authors in the same font and size as the first line (you may not make authors names smaller to save space.) Affiliations can be broken with a simple line break (\textbackslash  \textbackslash).
%\subsection{\LaTeX{} Copyright Notice}
%The copyright notice automatically appears if you use aaai20.sty. It has been hardcoded and may not be disabled.

%\subsection{Credits}
%Any credits to a sponsoring agency should appear in the acknowledgments section, unless the agency requires different placement. If it is necessary to include this information on the front page, use
%\textbackslash thanks in either the \textbackslash author or \textbackslash title commands.
%For example:
%\begin{quote}
%\begin{small}
%\textbackslash title\{Very Important Results in AI\textbackslash thanks\{This work is
% supported by everybody.\}\}
%\end{small}
%\end{quote}
%Multiple \textbackslash thanks commands can be given. Each will result in a separate footnote indication in the author or title with the corresponding text at the botton of the first column of the document. Note that the \textbackslash thanks command is fragile. You will need to use \textbackslash protect.

%Please do not include \textbackslash pubnote commands in your document.

%\subsection{Abstract}
%Follow the example commands in this document for creation of your abstract. The command \textbackslash begin\{abstract\} will automatically indent the text block. Please do not indent it further. {Do not include references in your abstract!}

%\subsection{Page Numbers}

%Do not \textbf{ever} print any page numbers on your paper. The use of \textbackslash pagestyle is forbidden.

%\subsection{Text }
%The main body of the paper must be formatted in black, ten-point Times Roman with twelve-point leading (line spacing). You may not reduce font size or the linespacing. Commands that alter font size or line spacing (including, but not limited to baselinestretch, baselineshift, linespread, and others) are expressly forbidden. In addition, you may not use color in the text. 

%\subsection{Citations}
%Citations within the text should include the author's last name and year, for example (Newell 1980). Append lower-case letters to the year in cases of ambiguity. Multiple authors should be treated as follows: (Feigenbaum and Engelmore 1988) or (Ford, Hayes, and Glymour 1992). In the case of four or more authors, list only the first author, followed by et al. (Ford et al. 1997).

%\subsection{Extracts}
%Long quotations and extracts should be indented ten points from the left and right margins. 

%\begin{quote}
%This is an example of an extract or quotation. Note the indent on both sides. Quotation marks are not necessary if you offset the text in a block like this, and properly identify and cite the quotation in the text. 

%\end{quote}

%\subsection{Footnotes}
%Avoid footnotes as much as possible; they interrupt the reading of the text. When essential, they should be consecutively numbered throughout with superscript Arabic numbers. Footnotes should appear at the bottom of the page, separated from the text by a blank line space and a thin, half-point rule. 

%\subsection{Headings and Sections}
%When necessary, headings should be used to separate major sections of your paper. Remember, you are writing a short paper, not a lengthy book! An overabundance of headings will tend to make your paper look more like an outline than a paper. The aaai.sty package will create headings for you. Do not alter their size nor their spacing above or below. 

%\subsubsection{Section Numbers}
%The use of section numbers in AAAI Press papers is optional. To use section numbers in \LaTeX{}, uncomment the setcounter line in your document preamble and change the 0 to a 1 or 2. Section numbers should not be used in short poster papers.

%\subsubsection{Section Headings.}
%Sections should be arranged and headed as follows: 

%\subsubsection{Acknowledgments.}
%The acknowledgments section, if included, appears after the main body of text and is headed ``Acknowledgments." This section includes acknowledgments of help from associates and colleagues, credits to sponsoring agencies, financial support, and permission to publish. Please acknowledge other contributors, grant support, and so forth, in this section. Do not put acknowledgments in a footnote on the first page. If your grant agency requires acknowledgment of the grant on page 1, limit the footnote to the required statement, and put the remaining acknowledgments at the back. Please try to limit acknowledgments to no more than three sentences. 

%\Subsubsection{Appendices.}
%Any appendices follow the acknowledgments, if included, or after the main body of text if no acknowledgments appear. 

%\subsubsection{References}
%The references section should be labeled ``References" and should appear at the very end of the paper (don't end the paper with references, and then put a figure by itself on the last page). A sample list of references is given later on in these instructions. Please use a consistent format for references. Poorly prepared or sloppy references reflect badly on the quality of your paper and your research. Please prepare complete and accurate citations.

%\subsection{Illustrations and Figures}
%Figures, drawings, tables, and photographs should be placed throughout the paper near the place where they are first discussed. Do not group them together at the end of the paper. If placed at the top or bottom of the paper, illustrations may run across both columns. Figures must not invade the top, bottom, or side margin areas. Figures must be inserted using the \textbackslash usepackage\{graphicx\}. Number figures sequentially, for example, figure 1, and so on. 

%The illustration number and caption should appear under the illustration. Labels, and other text with the actual illustration must be at least nine-point type. 

%If your paper includes illustrations that are not compatible with PDF\TeX{} (such as .eps or .ps documents), you will need to convert them. The epstopdf package will usually work for eps files. You will need to convert your ps files to PDF however.



%\subsubsection{Low-Resolution Bitmaps.}
%You may not use low-resolution (such as 72 dpi) %screen-dumps and GIF files---these files contain so few pixels that they are always blurry, and illegible when printed. If they are color, they will become an indecipherable mess when converted to black and white. This is always the case with gif files, which should never be used. The resolution of screen dumps can be increased by reducing the print size of the original file while retaining the same number of pixels. You can also enlarge files by manipulating them in software such as PhotoShop. Your figures should be 300 dpi when incorporated into your document.

%\subsubsection{\LaTeX{} Overflow.}
%\LaTeX{} users please beware: \LaTeX{} will sometimes put portions of the figure or table or an equation in the margin. If this happens, you need to scale the figure or table down, or reformat the equation.{ \bf Check your log file!} You must fix any overflow into the margin (that means no overfull boxes in \LaTeX{}). \textbf{Nothing is permitted to intrude into the margin or gutter.} 

%The most efficient and trouble-free way to fix overfull boxes in graphics is with the following command:

%\begin{quote}
%\begin{small}
%\textbackslash resizebox\{.95\textbackslash columnwidth\}{!}\{
%\}
%\end{small}\end{quote}

%Be certain, however, that your figures remain legible without magnification.

%\subsubsection{Using Color.}
%Use of color is restricted to figures only. It must be WACG 2.0 compliant. (That is, the contrast ratio must be greater than 4.5:1 no matter the font size.) It must be CMYK, NOT RGB. It may never be used for any portion of the text of your paper. The archival version of your paper will be printed in black and white and grayscale.The web version must be readable by persons with disabilities. Consequently, because conversion to grayscale can cause undesirable effects (red changes to black, yellow can disappear, and so forth), we strongly suggest you avoid placing color figures in your document. If you do include color figures, you must (1) use the CMYK (not RGB) colorspace and (2) be mindful of readers who may happen to have trouble distinguishing colors. Your paper must be decipherable without using color for distinction. 

%\subsubsection{Drawings.}
%We suggest you use computer drawing software (such as Adobe Illustrator or, (if unavoidable), the drawing tools in Microsoft Word) to create your illustrations. Do not use Microsoft Publisher. These illustrations will look best if all line widths are uniform (half- to two-point in size), and you do not create labels over shaded areas. Shading should be 133 lines per inch if possible. Use Times Roman or Helvetica for all figure call-outs. \textbf{Do not use hairline width lines} --- be sure that the stroke width of all lines is at least .5 pt. Zero point lines will print on a laser printer, but will completely disappear on the high-resolution devices used by our printers.

%\subsubsection{Photographs and Images.}
%Photographs and other images should be in grayscale (color photographs will not reproduce well; for example, red tones will reproduce as black, yellow may turn to white, and so forth) and set to a minimum of 300 dpi. Do not prescreen images.

%\subsubsection{Resizing Graphics.}
%Resize your graphics \textbf{before} you include them with LaTeX. You may \textbf{not} use trim or clip options as part of your \textbackslash includegraphics command. Resize the media box of your PDF using a graphics program instead. 

%\subsubsection{Fonts in Your Illustrations}
%You must embed all fonts in your graphics before including them in your LaTeX document.

%\subsection{References} 
%The AAAI style includes a set of definitions for use in formatting references with BibTeX. These definitions make the bibliography style fairly close to the one specified below. To use these definitions, you also need the BibTeX style file ``aaai.bst," available in the AAAI Author Kit on the AAAI web site. Then, at the end of your paper but before \textbackslash end{document}, you need to put the following lines:

%\begin{quote}
%\begin{small}
%\textbackslash bibliographystyle\{aaai\}
%\textbackslash bibliography\{bibfile1,bibfile2,...\}
%\end{small}
%\end{quote}

%Please note that you are required to use %\textbackslash bibliographystyle\{aaai\} for your references. You may not use named, plain, apalike, acm, ieeetr, siam, chicago, or any other style. Use of natbib is also not acceptable. (In addition to natbib, the aaai20.sty file is also incompatible with the hyperref and navigator packages. If you use either, your references will be garbled and your paper will be returned to you.) If you used natbib commands, an imprecise workaround is available (although it does not always work). You may put the following in your preamble (after removing \textbackslash usepackage\{natbib\}

%\begin{quote}\small
%\textbackslash newcommand\{\textbackslash %citet\}[1]\{\textbackslash %citeauthor\{\#1\}~\textbackslash shortcite\{\#1\}\}
%\textbackslash newcommand\{\textbackslash %citep\}\{\textbackslash cite\}
%\textbackslash newcommand\{\textbackslash %citealp\}[1]\{\textbackslash %citeauthor\{\#1\}~\textbackslash citeyear\{\#1\}\}
%\end{quote}


%References may be the same size as surrounding text. However, in this section (only), you may reduce the size to \textbackslash small if your paper exceeds the allowable number of pages. Making it any smaller than 9 point with 10 point linespacing, however, is not allowed. A more precise and exact method of reducing the size of your references minimally is by means of the following command: \begin{quote}
%\textbackslash fontsize\{9.8pt\}\{10.8pt\}
%\textbackslash selectfont\end{quote}

%\noindent You must reduce the size equally for both font size and line spacing, and may not reduce the size beyond \{9.0pt\}\{10.0pt\}.

%The list of files in the \textbackslash bibliography command should be the names of your BibTeX source files (that is, the .bib files referenced in your paper).

%The following commands are available for your use in citing references:
%\begin{quote}
%{\em \textbackslash cite:} Cites the given %reference(s) with a full citation. This appears as %``(Author Year)'' for one reference, or ``(Author %Year; Author Year)'' for multiple %references.\smallskip\\
%{\em \textbackslash shortcite:} Cites the given %reference(s) with just the year. This appears as %``(Year)'' for one reference, or ``(Year; Year)'' for %multiple references.\smallskip\\
%{\em \textbackslash citeauthor:} Cites the given %reference(s) with just the author name(s) and no %parentheses.\smallskip\\
%{\em \textbackslash citeyear:} Cites the given %reference(s) with just the date(s) and no %parentheses.
%\end{quote}



%Formatted bibliographies should look like the following examples.

%\smallskip \noindent \textit{Book with Multiple Authors}\\
%Engelmore, R., and Morgan, A. eds. 1986. \textit{Blackboard Systems.} Reading, Mass.: Addison-Wesley.

%\smallskip \noindent \textit{Journal Article}\\
%Robinson, A. L. 1980a. New Ways to Make Microcircuits Smaller. \textit{Science} 208: 1019--1026.

%\smallskip \noindent \textit{Magazine Article}\\
%Hasling, D. W.; Clancey, W. J.; and Rennels, G. R. 1983. Strategic Explanations in Consultation. \textit{The International Journal of Man-Machine Studies} 20(1): 3--19.

%\smallskip \noindent \textit{Proceedings Paper Published by a Society}\\
%Clancey, W. J. 1983. Communication, Simulation, and Intelligent Agents: Implications of Personal Intelligent Machines for Medical Education. In \textit{Proceedings of the Eighth International Joint Conference on Artificial Intelligence,} 556--560. Menlo Park, Calif.: International Joint Conferences on Artificial Intelligence, Inc.

%\smallskip \noindent \textit{Proceedings Paper Published by a Press or Publisher}\\
%Clancey, W. J. 1984. Classification Problem Solving. In \textit{Proceedings of the Fourth National Conference on Artificial Intelligence,} 49--54. Menlo Park, Calif.: AAAI Press. 

%\smallskip \noindent \textit{University Technical Report}\\
%Rice, J. 1986. Poligon: A System for Parallel Problem Solving, Technical Report, KSL-86-19, Dept. of Computer Science, Stanford Univ. 

%\smallskip \noindent \textit{Dissertation or Thesis}\\
%Clancey, W. J. 1979. Transfer of Rule-Based Expertise through a Tutorial Dialogue. Ph.D. diss., Dept. of Computer Science, Stanford Univ., Stanford, Calif.

%\smallskip \noindent \textit{Forthcoming Publication}\\
%Clancey, W. J. 2021. The Engineering of Qualitative Models. Forthcoming.

%For the most up to date version of the AAAI reference style, please consult the \textit{AI Magazine} Author Guidelines at \url{https://aaai.org/ojs/index.php/aimagazine/about/submissions#authorGuidelines}



%\section{Proofreading Your PDF}
%Please check all the pages of your PDF file. The most commonly forgotten element is the acknowledgements --- especially the correct grant number. Authors also commonly forget to add the metadata to the source, use the wrong reference style file, or don't follow the capitalization rules or comma placement for their author-title information properly. A final common problem is text (expecially equations) that runs into the margin. You will need to fix these common errors before submitting your file. 

%\section{Improperly Formatted Files }
%In the past, AAAI has corrected improperly formatted files submitted by the authors. Unfortunately, this has become an increasingly burdensome expense that we can no longer absorb (we are charged double for papers that require reformatting). Consequently, if your file is improperly formatted, it will probably be returned to you by the outside Production agency. If that happens, you will be required to fix your file and pay a resubmission fee.

%\subsection{\LaTeX{} 209 Warning}
%If you use \LaTeX{} 209 your paper will be returned to you unpublished. Convert your paper to \LaTeX{}2e.

%\section{Naming Your Electronic File}
%We require that you name your \LaTeX{} source file with the last name (family name) of the first author so that it can easily be differentiated from other submissions. Complete file-naming instructions will be provided to you in the submission instructions.

%\section{Submitting Your Electronic Files to AAAI}
%Instructions on paper submittal will be provided to you in your acceptance letter.

%\section{Inquiries} 
%If you have any questions about the preparation or submission of your paper as instructed in this document, please contact AAAI Press at the address given below. If you have technical questions about implementation of the aaai style file, please contact an expert at your site. We do not provide technical support for \LaTeX{} or any other software package. To avoid problems, please keep your paper simple, and do not incorporate complicated macros and style files.

%\begin{quote}
%\noindent AAAI Press\\
%2275 East Bayshore Road, Suite 160\\
%Palo Alto, California 94303\\ 
%\textit{Telephone:} (650) 328-3123\\ 
%\textit{E-mail:} See the submission instructions for %your particular conference or event.
%\end{quote}

%\section{Additional Resources}
%\LaTeX{} is a difficult program to master. If you've used that software, and this document didn't help or some items were not explained clearly, we recommend you read Michael Shell's excellent document (testflow doc.txt V1.0a 2002/08/13) about obtaining correct PS/PDF output on \LaTeX{} systems. (It was written for another purpose, but it has general application as well). It is available at www.ctan.org in the tex-archive.

%\section{ Acknowledgments}
%AAAI is especially grateful to Peter Patel Schneider %for his work in implementing the aaai.sty file, %liberally using the ideas of other style hackers, %including Barbara Beeton. We also acknowledge with %thanks the work of George Ferguson for his guide to %using the style and BibTeX files --- which has been %incorporated into this document --- and Hans Guesgen, %who provided several timely modifications, as well as %the many others who have, from time to time, sent in %suggestions on improvements to the AAAI style. %
%
%The preparation of the \LaTeX{} and Bib\TeX{} files that implement these instructions was supported by Schlumberger Palo Alto Research, AT\&T Bell Laboratories, Morgan Kaufmann Publishers, The Live Oak Press, LLC, and AAAI Press. Bibliography style changes were added by Sunil Issar. \verb+\+pubnote was added by J. Scott Penberthy. George Ferguson added support for printing the AAAI copyright slug. Additional changes to aaai.sty and aaai.bst have been made by the AAAI staff.

%\bigskip
%\noindent Thank you for reading these instructions carefully. We look forward to receiving your electronic files!















A common use case of crowdsourcing is to enable businesses to complete, through the help of crowd workers, tasks that artificial intelligence alone cannot accomplish \cite{}. 

Crowdsourcing can make this promise because they utilize algorithms and interfaces that eliminate the expenses of searching for, matching, training/retaining, and communicating with workers \cite{}. 

practical
functions such as sourcing, scheduling, shipping, and billing


On-demand platforms disrupt the burden of hiring by providing APIs to handle practical
functions such as sourcing, scheduling, shipping, and billing

While transaction costs are traditionally thought to be incurred by corporations,
with the on-demand economy—in which management is partially offloaded to algorithms and
platforms—some of these transaction costs are passed on to clients and freelancers [10].


Research has suggested, that firms can reduce their costs when using Crowdsourcing to solve a task 

In using opening innovation processes and permitting for co-development, it has been suggested, that firms can reduce their costs when using Crowdsourcing to solve a task 


At the heart of crowdsourcing is the assumption that crowdsourcing will reduce transaction costs, and the profits of companies will be increased. The concept of transactional costs has its beginnings in current economic theory and refers to \emph{``expenses associated with managing the production and exchange of goods or services''}\cite{}. 

all these have their beginnings in current economic theory.

Crowdsourcing can make this promise because they utilize algorithms and interfaces that eliminate the expenses of searching for, matching, training/retaining, and communicating with workers \cite{}. 

e. On-demand platforms disrupt the burden of hiring by providing APIs to handle practical
functions such as sourcing, scheduling, shipping, and billing

Originating in economic theory [37], the
concept of transaction costs refers to “expenses associated with managing the production of goods
and services” [10]. While transaction costs are traditionally thought to be incurred by corporations,
with the on-demand economy—in which management is partially offloaded to algorithms and
platforms—some of these transaction costs are passed on to clients and freelancers [10].


Several researchers have pointed out that using Crowdsourcing to solve tasks can be cheaper than solving them internally. This is also a key argument in TCT, which proposes that firms need to reduce costs to raise their profitability while maintaining their competitive advantage

Among the key arguments of transaction cost theory is the need to reduce costs to improve profitability and maintain competitiveness (Coase, 1937). In using opening innovation processes and permitting for co-development, it has been suggested, that firms can reduce their costs when using Crowdsourcing to solve a task (Howe, 2009, Howe, 2016). PharmaFX conducted Crowdsourcing to get scientific inputs. The question is whether PharmaFX's Crowdsourcing Challenge was economically viable compared to internal alternatives.



















Crowdsourcing markets serve the purpose of being platforms that enable businesses to access crowd workers and integrate their work seamlessly into the businesses' services. A common use case of crowdsourcing is to enable businesses to complete, through the help of crowd workers, tasks that artificial intelligence alone cannot accomplish. 
Crowdsourcing comes with the added expectation that the incorporation of crowd work will not increase the costs for businesses by too much. Crowd markets have even gone a step further and have additionally promised to reduce businesses' costs. 
% SS: If they have promised the above could you add a quote or a citation? If they haven't made this promise just cut the previous sentence.
Crowdsourcing markets can make this promise because they utilize algorithms and interfaces that eliminate the expenses of searching for, matching, training/retaining, and communicating with workers. 















While being able to hire humans in this way can be faster and more efficient for companies than using traditional methods, all of the transaction costs have not actually disappeared. Many argue that the transaction costs have simply shifted from the shoulders of companies onto the shoulders of workers in the form of invisible labor. But, we currently know little about how much time workers spend doing this invisible labor actually and how much it costs them.  

In this paper, we combine survey and large scale log data to examine invisible labor on Amazon Mechanical Turk.  We record the amount of time that XX workers on Amazon Mechanical Turk dedicate to invisible labor. We find that workers on average spent XX hrs daily on invisible labor. XX was the type of invisible labor that took the most time (XX hrs a day on average). We also investigate the type of work practices that crowd workers adopt to minimize how much time they invest in invisible labor, examples include XX. Together, our results start to reveal the larger implications for crowdsourcing markets of the continuing invisibility of labor and helps to inform designers on how to create more worker-centric platforms and tools. We hope that through our paper, the invisible labor in crowdsourcing markets will become more visible. 



%
%A main promise of crowd work is that it can cut labor costs by eliminating the expenses of searching for, training, and communicating with workers. The promise of cutting costs and thus increasing the profits for companies has lead crowd work to become widely popular. However, 
 
 
 
 
 
 
 
 
 
 
 
 we survey XX crowd workers on Amazon Mechanical Turk and ask them to estimate the amount of time they spend on different types of invisible labor, and then compare estimates to the actual time crowd workers spend on different types of invisible labor.



examine the practices that crowd workers have developed to try to minimize the amount of invisible labor they do. 






We also studied how much workers' felt that their practices for reducing time spe
and whether they felt that their p



We then quantify the uncertainty in audience size by investigating actual audience information for 220,000 Facebook
users. We examine whether there are reasonable heuristics
that users could adopt for estimating audience size for a specific post, for example friend count or feedback, or whether
the variance is too high for users to use those signals reliably.
We then test the same heuristics for estimating audience size
over a one-month period


This paper investigates users’ perceptions of their invisible
audience, and the inherent uncertainty in audience size as a
limit for users’ estimation abilities. We survey active Facebook users and ask them to estimate their audience size, then
compare their estimates to their actual audience size using
server logs. We examine the folk theories that users have developed to guide these estimates, including approaches that
reverse-engineer viewership from friend count and feedback.

We then quantify the uncertainty in audience size by investigating actual audience information for 220,000 Facebook
users. We examine whether there are reasonable heuristics
that users could adopt for estimating audience size for a specific post, for example friend count or feedback, or whether
the variance is too high for users to use those signals reliably.
We then test the same heuristics for estimating audience size
over a one-month period.

We found that employee clients most often hired freelancers to save time rather than money. However, in exchange for those time savings, they had
one major concern and they took on two major transaction costs. Their concerns stemmed from
power asymmetries between themselves and the freelancers—in other words, clients have more
influence over the actions of freelancers than freelancers do over clients. (For example, both clients
and freelancers are rated by one another, but poor ratings are perceived as more consequential
for freelancers than they are for clients [22, 35].) As a result, their main concern was how to work
with a freelancer responsibly. They had to navigate mitigating risk for the company (e.g., intellectual property risk and employee classification risk) and their own sense of ethical responsibility
to freelancers. We found that they sometimes feared the potential “race to the bottom” that the
freelance economy might enable, and thus they wanted their corporation to provide guardrails and
guidelines about responsible use of the freelance economy












%occur within the context of paid employment that workers perform in response to requirements
%(either implicit or explicit) from employers and that are crucial for
%workers to generate income, to obtain or retain their jobs, and to further their careers, yet are often overlooked, ignored, and/or devalued by
%employers, consumers, workers, and ultimately the legal system itself.

%First, work that is not seen is not valued, either symbolically or
%materially. Second, if workers themselves do not see their efforts as valuable work, they are less likely to organize, appeal for public support,
%or challenge their working conditions through the legal system. Even if
%they want to mobilize, the invisibility of their work—and in many cases,
%of the workers themselves—may make it difficult for them to gain political traction or support from consumers. Finally, and most crucially, if
%the state and legal systems do not acknowledge the labor, it will not be
%addressed in policy and law. A prominent theme running throughout
%this book is how invisible labor is often unregulated.

%In other scholarship addressing the concept of hidden labor within the
%context of paid employment, invisibility has typically been associated
%with minimum-wage jobs or the underground economy



%We balance our perspective to account for a range of occupational positions that include the
%middle and professional strata of the workforce. Our authors consider
%the role of affluent or middle-class workers in retail; the increasing use
%of unpaid internships that are disproportionately available to collegeeducated, economically privileged students; and the status of skilled
%knowledge workers on the Internet

%what counts as work, and why are
%some forms of work invisible? We focus on forms of labor that occur
%within formal employment relationships but are not conceptualized as
%work and so remain hidden from view—sometimes in the public imagination, sometimes from consumers, and sometimes from the workers
%themselves. When their work is erased, the workers themselves are
%sometimes rendered invisible as well. We ask what forces and trends are
%preventing employers, consumers, and employees from “seeing” the
%work that is done and blocking regulators and policy makers from
%addressing its impact

%Given that there are in general no legal requirements to make job postings, workers have to ensure they are not working for businesses who are trying to harvest their emails, do identify theft, or even get them to do illegal activity. Interview studies have showcased that having to develop a hyper-vigilance is not only causing unnecessary stress in crowd workers, it is also creating economical losses to workers. The time they have to invest in being vigilant over who they work with is time that 

%Posting to a social network site is like speaking to an audience from behind a curtain. The audience remains invisible
%to the user: while the invitation list is known, the final attendance is not. Feedback such as comments and likes is the
%only glimpse that users get of their audience. That audience
%varies from day to day: friends may not log in to the site
%may not see the content, or may not reply. While established
%media producers can estimate their audience through surveys,
%television ratings and web analytics, social network sites typically do not share audience information. This design decision
%has privacy benefits such as plausible deniability, but it also
%means that users may not accurately estimate their invisible
%audience when they post content.

There are several definitions on what invisible labor is. We take the definition from \cite{} that defined invisible labor within contemporary contexts and included gig work. They defined invisible labor 









At the core of crowd markets are the promises that crowd work (i.e., the main service that crowd markets offer) will enable businesses to complete work that artificial intelligence alone cannot do, and that the integration of this work will not increase the costs of businesses. To appeal even more to businesses, crowd markets have gone a step further and promised to even reduce businesses' costs. This is enabled allegedly through algorithms and computational interfaces that remove businesses' expensive costs of searching, matching, training, communicating, or retaining workers. 








%%
%% The code below is generated by the tool at http://dl.acm.org/ccs.cfm.












%% Please copy and paste the code instead of the example below.
%%“expenses associated with managing the production of goods
%and services”


%% A "teaser" image appears between the author and affiliation
%% information and the body of the document, and typically spans the
%% page.
%\begin{teaserfigure}
%  \includegraphics[width=\textwidth]{sampleteaser}
%  \caption{Seattle Mariners at Spring Training, 2010.}
%  \Description{Enjoying the baseball game from the third-base
%  seats. Ichiro Suzuki preparing to bat.}
%  \label{fig:teaser}
%\end{teaserfigure}

%%
%% This command processes the author and affiliation and title
%% information and builds the first part of the formatted document.
\maketitle





















recent interviews with crowd workers hint that 
 (labor which workers have to do, but for which they are not paid)












%begin to reveal the invisible undercurrents
%of audience attention and behavior in online social networks.
%Our analysis helps to inform designers on how to create more worker centric platforms and tools. 



%One of the main promises of crowd work is that it can cut the costs associated with completing labor. Particularly, by eliminating the expenses of searching, matching, training, and communicating with workers.  
%One of the premises of crowd work is that it reduces labor costs by eliminating the and therefore increases the profits of companies and employers who use crowd labor. Crowd work advertises that it by eliminating the friction
%and therefore increases the profits of companies and employers who use crowd labor. Crowd work has historically been known to push uneven work and power dynamics between workers and employers. Crowd workers not only have little bargaining power, but a great portion of the costs associated with completing the labor have shifted ontocosts of getting the work done have shifted to workers. 


%One of the main promises of crowd work is that it can cut labor costs by eliminating the expenses associated with searching, matching, training, and communicating with workers. The promise of cutting costs and thus increasing the profits of companies and employers has lead crowd work to become widely popular. However, the costs have not actually disappeared; they have simply shifted from the shoulders of companies and employers onto the shoulders of workers in the form of invisible labor. We currently know little about how much invisible labor costs crowd workers.  In this paper, we combine survey and large scale log data to examine the invisible labor of crowd workers on Amazon Mechanical Turk.  We recorded the amount of time that XX workers on Amazon Mechanical Turk dedicated to invisible labor. We found that workers on average spent XX hours a day on invisible labor. XX was the type of invisible labor that took the most time (XX hours a day on average). We also investigated the type of work practices that helped workers minimize how much they invested in invisible labor.  Together, our results start to reveal the implications of invisible labor on crowd markets, and help to inform designers on how to create more worker centric platforms and tools. 
